ProLoc: Robust Location Proofs in Hindsight

Many online services rely on self-reported locations of user devices like smartphones. To mitigate harm from falsified self-reported locations, the literature has proposed location proof services (LPSs), which provide proof of a device's location by corroborating its self-reported location using short-range radio contacts with either trusted infrastructure or nearby devices that also report their locations. This paper presents ProLoc, a new LPS that extends prior work in two ways. First, ProLoc relaxes prior work's proofs that a device was at a given location to proofs that a device was within distance "d" of a given location. We argue that these weaker proofs, which we call "region proofs", are important because (i) region proofs can be constructed with few requirements on device reporting behavior as opposed to precise location proofs, and (ii) a quantitative bound on a device's distance from a known epicenter is useful for many applications. For example, in the context of citizen reporting near an unexpected event (earthquake, violent protest, etc.), knowing the verified distances of the reporting devices from the event's epicenter would be valuable for ranking the reports by relevance or flagging fake reports. Second, ProLoc includes a novel mechanism to prevent collusion attacks where a set of attacker-controlled devices corroborate each others' false locations. Ours is the first mechanism that does not need additional infrastructure to handle attacks with made-up devices, which an attacker can create in any number at any location without any cost. For this, we rely on a variant of TrustRank applied to the self-reported trajectories and encounters of devices. Our goal is to prevent retroactive attacks where the adversary cannot predict ahead of time which fake location it will want to report, which is the case for the reporting of unexpected events.

==> src_arXiv/data-artifacts.tex <==
\section{Dataset and artifact removal}
\label{sec:data-arifacts}

\input{src/loc-opt}



==> src_arXiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

Location-based services are sensitive to users' current or past
locations.  Examples include navigation, ride-hailing, and car-sharing
services, social networks,
dating services~\cite{happn}, fitness apps~\cite{fitbit}, and certain
health-related apps~\cite{korea_apps}.
A well-known challenge for these services is the relative ease with
which either mobile platform software, app, or users can report an
incorrect location.

Such attacks can undermine the integrity of location-based services.
For instance, drivers of ride-hailing services (Uber, Lyft) have
reported journeys that did not take place to increase their
income~\cite{uberattack, spoof_uber}; users have abused social networks to get
notifications about people or resources that are not actually
nearby~\cite{fakelocation}.
Furthermore, attackers have targeted mobile mapping services (Google
Maps, Waze) to generate fake traffic information and congestion
spots~\cite{wang2018ghost,gmapattack, raponi2020fridges}.

{\em Location proofs}\footnote{A location proof is not a proof
  in the strict mathematical sense of the word. We use the term because it is already used
  in the literature.}  can
add robustness to location-based services.  For instance,
crowd-sourced sensor readings, incident reports, and audio-visual
material can be reliably tagged with the locations where they were
captured, and users can prove that they actually visited events,
restaurants, or hotels they submit reviews for.  Saroiu et
al.~\cite{saroiu2009enabling} note that location proofs can also
enable robust new services like verified loyalty programs, green
community, restricted-access content delivery, reducing review and
auction fraud, and verifying residency requirements.
  
Prior work has considered various location proof
systems~\cite{saroiu2009enabling,veriplace,Hasan2011WhereHY,crepuscolo,applaus,link,stamp,globalattestation}.
Some rely on WiFi base stations, while others use nearby devices in
Bluetooth range as witnesses to produce location proofs.  All existing
systems minimize the information provided to the system in the
interest of privacy. For instance, location proofs
are available only when witnesses are available at the
precise time in question, and must be produced {\em a priori} if and
when a subsequent need for them is foreseen. We contend that data
minimization comes at the expense of flexibility on the one hand, and
robustness to collusion attacks on the other. Regarding flexibility,
even if witnesses were present, a proof cannot be generated
for a location or trajectory segment retroactively unless the need was
foreseen; moreover, conservatively generating a proof for all
  witnessed locations is infeasible due to computational and energy
  costs.  Regarding robustness, no existing system is robust to
large-scale attacks where an adversary invents fictitious devices and
trajectories.

In this work, we choose a different point in the design space and
describe {\em \sys}, a location-proof system in which devices
regularly upload locations and received BLE adverts to a secure backend
as a matter of course.
This enables \emph{retroactive proofs} that
the device's location at any given time in the past lies within a
\emph{feasible region} whose shape depends on the density and diversity
of encounters the device had around the time.
Moreover, \sys\ can derive the feasible region in a principled manner
from the set of encounters a device had around the time in question,
and the topology of the transportation network.
Additionally, the rich data collection enables {\em defenses
    against a large class of collusion attacks involving fictitious
  devices},
i.e., trust computations based on devices' interconnectivity.

\sys\ derives much of its power from aggregating and
  processing the contact and mobility data of many devices. To secure
  this sensitive data, \sys\ uses end-to-end encryption and its backend computes
  on data inside a trusted execution environment (TEE). A TEE ensures
  that data can be decrypted only within a hardware-isolated domain
  that runs the approved and validated \sys\ software.

\sys\ provides location proofs without
  geo-distri\-buted trusted infrastructure such as trusted WiFi base stations, which would be expensive to install and
  operate and hard to secure. Without such
  infrastructure, however, a general defense against collusion attacks (that enable an adversary to create fake location proofs)
  does not exist, and may be impossible in cases where the adversary
  has a device present at the target location.  \sys\ takes an
  important step by offering the first effective defense against a
  large class of easy-to-mount collusion attacks involving a large
  number of fictitious and a limited number of physical devices
  controlled by the adversary.  The current design is limited to {\em
    retroactive} attacks, where the adversary cannot predict upfront
  for what time and location it wishes to generate a false proof. An
  extension to {\em premeditated} attacks remains as future work.  

Our contributions include:
(i) a principled technique to compute the feasible region within which
a device could have plausibly resided at a past instant, given the
set of encounters the device had around that instant and the topology
of the transportation network (\cref{sec:loc-conf});
(ii) a comprehensive analysis of collusion attacks against location
proof systems (\cref{sec:attacks-sys});
(iii) a defense against {\em retroactive} collusion attacks involving
an unlimited number of fictitious devices, a bounded number of corrupt
devices, as well as multiplicity (Sybil) attacks; we also sketch
possible defenses to {\em premeditated} collusion attacks
(\cref{sec:dev-trust});
(iv) the design and implementation of a location-proof system based on
these ideas (\cref{sec:service,sec:dev-trust}); and
(v)
 an experimental evaluation based on the real-world DTU dataset of
locations and BLE contacts collected from 850 devices over a period of
3 years (\cref{sec:eval}).




  



  



==> src_arXiv/loc-confidence.tex <==
\subsection{Feasible Region Computation}
\label{sec:loc-conf}




In this section, we describe how {\sys} computes the feasible region
for a device $\device$ at time $t$ with robustness $N$.



\btitle{Peer selection algorithm.} 
Suppose that device $d$ had and encounter $E_{d,d_A,t_{e,A}}$ with device $d_A$ at time $t_{e,A}$. Let $\locc_{A}$ and $\locc_{A'}$ be the self-reported reported locations of device $d_A$ preceding and following $t_e$ in $d_A$'s history and let these be at times $t_A$ and $t_A'$, respectively.
For each encounter $E_{d,d_A,t_{e,A}}$ that device $d$ had, we compute a function, $f$, defined as
\begin{equation*}
f = (|t_e - t|) + min(|t_e - t_A|, |t_e - t_A'|) +  \frac{D \left(\locc - \locc_{min(tA, tA')}\right)}{v_{avg}} ,
\end{equation*}
where $D$ is a function that computes the geographical distance between $\locc$ and $\locc_{min(tA, tA')}$. We use function $f$ to select, among all the encounters that a user had around time $t$ and position $\locc$, the ones for which peers have reported positions that are both close, in time, with $t_e$ and spatially adjacent to $\theta$. 
We then pick the first $N+1$ of these encounters with distinct peers.

\btitle{Feasible region computation.}We describe the feasible region computation for $N = 0$ before the general case.

\btitle{Case $N = 0$.}  In this case, all encounter peers of
$\device$ are assumed to be legitimate -- their location and encounter
reports are correct. To compute a feasible region for $\device$ at
time $t$ and location $\locc$ under this assumption, {\sys} selects, using function $f$, an encounter of
$\device$ close to time $t$. This single encounter constitutes the
quorum. Suppose the encounter happened at time $t_{e,A}$ and the encounter
peer is device $\device_A$. Let $\locc_A$ and $\locc_A'$ be the
self-reported locations of $\device_A$ preceding and following $t_{e,A}$
in $\device_A$'s history and let these be at times $t_A$ and $t_A'$,
respectively.

We start from the first location report, $\locc_A$, at time $t_A$, and
determine a feasible region $\regionof{\device_A}{t_{e,A}}$ for
$\device_A$ (not $\device$) at the time of the encounter, $t_{e,A}$. Since
$A$ was at $\locc_A$ at time $t_A$, this region is simply
$\regionof{A}{t_{e,A}} = \api{isochrone}(\{\locc_A\}, |t_{e,A} - t_A|)$.

Next, we compute a feasible region $\regionof{\device}{t_{e,A}}$ for
$\device$ at time $t_{e,A}$ (not $t_A$). Since $\device$ encountered
$\device_A$ at this time, $\device$ must have been within bluetooth
range, say $r_{BLE}$ meters, of $\device_A$. Hence,
$\regionof{\device}{t_{e,A}}$ is obtained by expanding the region
$\regionof{\device_A}{t_{e,A}}$ on the map by $r_{BLE}$
meters.\footnote{Our current implementation uses a conservative value
  $r_{BLE} = 100$m. This value can be reduced by measuring effective
  BLE range at different places on the map empirically.}

Using this, we compute a feasible region $\region$ for $\device$ at
time $t$ as $\region = \api{isochrone}(\regionof{\device}{t_e}, |t -
t_{e,A}|)$.

We now repeat this process with $\device_A$'s second self-reported
location $\locc_A'$ at time $t_A'$. This yields a second feasible
region $\region'$ for $\device$ at time $t$.

Since $\device$'s location at time $t$ is constrained by both
$\region$ and $\region'$, the final feasible region for $\device$ at
time $t$ is the \emph{intersection} of the two, i.e., $\region
\mathrel{\cap} \region'$. 

\btitle{General $N$.}  Next, we describe the computation of
a feasible region for $\device$ at time $t$ and location $\locc$ for a non-zero $N$. Here,
up to $N$ of $\device$'s encounter peers may be adversary controlled,
so we pick, using function $f$, a quorum of $N+1$ encounters of $\device$ close to
time $t$ with \emph{distinct peers}.

Using each of the $N+1$ encounters, we compute a feasible region for
$\device$ as in the case $N=0$. The required feasible region is then
the \emph{union} of these feasible regions. By assumption, one of the
$N+1$ devices in the quorum honestly, so $\device$ must have been
located in this union at time $t$.

Figure~\ref{fig:conf-region} summarizes the entire calculation of the
feasible region in pseudocode.


\begin{figure}
  \begin{tabular}{l}
    \hline
    API call $\api{feasible\_region}(\device,\locc, t, N)$ \\
    \hline
    ;; $\api{D}$ is {\sys}'s internal database.\\
    ;; $\api{Map}$ is the map service.\\
    \\
    ;; Compute feasible region w.r.t.\ a single peer location\\
    $\kw{function}$ $\api{region\_peer\_report}(t_e, t_A, \locc_A)$: \\
    \ptab $\regionof{\device_A}{t_e} \leftarrow \api{Map.isochrone}(\{\locc_A\}, |t_e - t_A|)$ \\
    \ptab $\regionof{\device}{t_e} \leftarrow \api{Map.grow\_region}(\regionof{\device_A}{t_e}, r_{BLE})$ \\
    \ptab $\region \leftarrow \api{Map.isochrone}(\regionof{\device}{t_e}, |t - t_e|)$ \\
    \ptab $\kw{return} ~\region$\\
    \\
    ;; Compute feasible region w.r.t.\ a single encounter\\
    $\kw{function}$ $\api{region\_encounter}(E)$: \\
    \ptab $\device_A \leftarrow E.\api{other\_peer}(\device)$ \\
    \ptab $t_e \leftarrow E.\api{timeof}()$ \\
    \ptab $(\locc_A, t_A) \leftarrow \api{D.prev\_location\_report}(\device_A, t_e)$ \\
    \ptab $(\locc_A', t_A') \leftarrow \api{D.next\_location\_report}(\device_A, t_e)$ \\
    \ptab $\region \leftarrow \api{region\_peer\_report}(t_e, t_A, \locc_A)$ \\
    \ptab $\region' \leftarrow \api{region\_peer\_report}(t_e, t_A', \locc_A')$ \\
    \ptab $\kw{return} ~(\region \mathrel{\cap} \region')$\\
    \\
    ;; Top level code \\
    $\{E_1, \ldots, E_{N+1}\} \leftarrow \api{D.encs\_distinct\_peers}(\device,\locc, t, N+1)$\\
    $\kw{for} ~i = 1 ~ \kw{to} ~ (N+1)$:\\
    \ptab $R_i \leftarrow \api{region\_encounter}(E_i)$\\
    $\kw{return} ~(R_1 \mathrel{\cup} \ldots \mathrel{\cup} R_{N+1})$\\
    \hline
  \end{tabular}
  \caption{Feasible region computation}
  \label{fig:conf-region}
\end{figure}


\btitle{Refining the feasible region.}  We can \emph{refine}
the feasible region at the expense of more computation by picking $K$
distinct quorums of $N+1$ encounters each (in the case $N=0$, just
picking $K$ different encounters). For each of these $K$ quorums, we
get a feasible region as described above. Since $\device$'s location
at time $t$ is in each of these feasible regions, it is also in their
\emph{intersection}, which is a smaller feasible region.

Since isochrone computation is expensive, our current implementation
performs this refinement only for $N = 0$. For higher $N$, it uses
only one quorum of $N+1$ encounters, but it picks this quorum
carefully. 

\textbf{Feasible region size.} Function $f$ selects encounters, and therefore peers, in such a way that, assuming that the street network around $\theta$ does not present rough discountinuities, minimize the area of the feasible region obtained considering $E_{d,d_A,t_{e,A}}$, and the distance between the resulting intersection and the location $\locc$ provided by $\device$ at time $t$.The size of feasible region is largely determined by two factors. First, higher $N$ result in larger, but
more robust feasible regions. Second, for a given $N$, the feasible
region size changes inversely with the density of $\device$'s
encounters in the vicinity of time $t$ and the density of location
reports by $\device$'s encounter peers in the vicinity of those
encounters. {\sys} returns more useful location proofs (i.e., smaller
feasible regions) in areas where encounters are dense and devices
report locations frequently. We explore the effect of changing $N$ and
changing density on feasible region size empirically in
Section~\ref{sec:eval-feasible-regions}.


==> src_arXiv/loc-opt.tex <==

\label{sec:loc-opt}

In this section, we describe how we can reduce noise in trajectories
reported by devices. Noise can originate from errors in the
  recorded locations and times, and can arise, for instance, when a
  GPS receiver looses synchronization due to poor reception indoors or
  due to line-of-sight obstructions.

Intuitively, the reported trajectories of two devices that
  report an encounter must coincide within BT range at the time of the
  encounter. Moreover, individual trajectories must be physically
  plausible, i.e., they cannot exceed practical speeds.  We can use
  these constraints to reduce noise in the recorded locations.  We
  perform this noise reduction on our location data after the artifact
  removal, which is specific to our dataset. However, the noise
  reduction can and should be performed also on location data in a
  live \sys\ deployment.

The inputs to the noise reducing computation are the self-reported
trajectories of all devices and the encounters between them (denoted
$\allencs$). Using these inputs, we set up an \emph{optimization
problem} that penalizes violation of physical constraints --
unrealistic travel speeds and out-of-BLE-range encounters. We then
solve this optimization problem to obtain a corrected coordinate for
every location report in the input. These corrected coordinates,
called the \emph{consolidated coordinates}, are the output of this
intermediate step.



==> src_arXiv/optimization.tex <==

\subsection{Optimization}
\label{sec:optimization}

\sys~ combines users' GPS location recordings and Bluetooth pairwise encounter histories to estimate a more accurate position for each user at each point in time. Such adjustments address both GPS inaccuracies and potential, deliberate manipulations of a user device's trajectory.

Let $\mathcal{D}$ be the set of user devices in our dataset, which contains:
\begin{itemize}
\item A set of GPS reported locations:
\begin{center}
$\mathcal{L} = \{ (d_i, t_i, \boldsymbol{\theta_i}, a_i)  \}$
\end{center}
Where $d \in \mathcal{D}$, $t$ is a timestamp, $\boldsymbol{\theta}$ is a pair of geographical coordinates, and $a$ is the self-reported GPS accuracy.
\item A set of pairwise Bluetooth encounters:
\begin{center}
$\mathcal{B} = \{ (d_i, p_i, t_i) \}$
\end{center}
Where $d, p \in \mathcal{D}$ represent the device ids of a user and their encounter peer, respectively.
\end{itemize}
Depending on the particular choice of encounter formation protocol, which is independent from our system, a user device might either take an additional location recording when registering an encounter or not. In the following, we consider the general, worst-case assumption that an encounter entry does \textit{not} refer to a location recorded where the encounter took place. Thus, the optimization algorithm requires a pre-processing step, which we describe next.

